sZoom: A Framework for Automatic Zoom into High Resolution Surveillance Videos

Current cameras are capable of recording high resolution video. While viewing on a mobile device, a user can manually zoom into this high resolution video to get more detailed view of objects and activities. However, manual zooming is not suitable for surveillance and monitoring. It is tiring to continuously keep zooming into various regions of the video. Also, while viewing one region, the operator may miss activities in other regions. In this paper, we propose sZoom, a framework to automatically zoom into a high resolution surveillance video. The proposed framework selectively zooms into the sensitive regions of the video to present details of the scene, while still preserving the overall context required for situation assessment. A multi-variate Gaussian penalty is introduced to ensure full coverage of the scene. The method achieves near real-time performance through a number of timing optimizations. An extensive user study shows that, while watching a full HD video on a mobile device, the system enhances the security operator's efficiency in understanding the details of the scene by 99% on the average compared to a scaled version of the original high resolution video. The produced video achieved 46% higher ratings for usefulness in a surveillance task.

==> additional-papers.tex <==
\section{Additional Papers}  
In this section we provide a tabular comparison of our work with previous works. First we highlight the differences, and then we state how these difference make us better.




Ascendent Video Analysis: vision-based company offering products for target counting, intrusion detection, object classification, abondened baggage detection, dwelling etc.


In \cite{gaddam2015cameraman}, the authors automatiz zoom for  panoramic sports video. The RoI is determined on tracking the ball or selected player. The framework is not application for surveillance because: (1) we do not know what to track in advance (2) coverage and context are important which are ignored (3) The RoI adaptation is necessary for natural viewing which is missing (4) no fusion framework.

In \cite{chen2016learning}, the authors use recurrent decision trees for smooth trajectory prediction in sports videos. The smooth trajectory reduces jitter in the automatic camera motion.   

In \cite{wang2015wireless}, the authors propose multicast framework for zoomable video. The work is useful in our framework to extend to multiple users. The RoI is manually selected by the users and there is no automatic zoom. 

In \cite{zhai2015object}, the authors propose object detection by analyzing dense trajectories. It can be integrated easily in our sensitivity detection framework. 

In \cite{lim2014isurveillance}, the authors detect multiple events in different RoIs of the video. This work could be used to adapt the zoom time window (which is currently 5 second) according to the type of event. As the current automatic zoom is aimed to assist the security operator, we detect RoI based on low-level processing and leave the high level understanding to the operator. 

In \cite{zhu2012face} and \cite{li2015convolutional} the authors propose more robust face detection algorithms. Although the accuracy of face detector is very low in current framework, with the new advanced detectors the accuracy would increase. 

In \cite{pang2011classx}, the authors propose a framework to stream video lectures to mobile devices. The user can pan/tilt/zoom onto the streamed video. Once an RoI se selected y the user, the system tracks the RoI in the video until the user selected another RoI. There is not automatic zoom. 

In \cite{carlier2011combining}, the authors use saliency and motion to estimate the regions containing humans. We directly use human detector. Once RoI is detected, the authors recommend the RoI to the user. There is no automatic zoom. sZoom framework is modular in the sense new content analysis techniques can be easily plugged in the fusion step.

In \cite{shafiei2012jiku}, the Jiku live allows user to manually zoom and pan into the real-time video. This is not sufficient for surveillance because, once zoomed in, the user cannot see other parts of video which may contain  sensitive activities going on. Also, it is tiring to continuously keep zooming into different regions using finger gestures. The work does not propose any automatic zoom framework. 

In \cite{koccberber2014video}, the authors crop certain region of the video based on visual saliency and motion. The goal is video retargetting, no automatic zoom framework proposed. 


==> related-work.tex <==
\section{Related Works}  
In this section we provide a tabular comparison of our work with previous works. First we highlight the differences, and then we state how these difference make us better.

We could compare the earlier works with respect to the following points:
\begin{itemize}
\item \textbf{Online or not?} In surveillance systems we do not have full video before-hand. So the methos should be applicable online. 
\item \textbf{Context preserved or not?} Security operators need the surrounding context for situation assessment.
\item \textbf{Sensitivity criteria?} The sensitivity criteria should be based on surveillance tasks. 
\item \textbf{Content modification?} In surveillance scenario, content modification is not desired. 
\item \textbf{User input} Some regions may have a lot of motion, but still not important for surveillance. For example vehicle on the road. System should integrate this information in the sensitivity map.
\item \textbf{Region tracking?} After selecting the zoom region, the object may move. Therefore, we need to track the object and adjust window size. 
\end{itemize}


\begin{table*}
	\centering
		\caption{Summary of previous works.} 
		\centering
		\begin{tabular}{p{2cm}|p{2cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{1.5cm}|p{2cm}}
			\hline
			Previous Work &  Online or not? & Context preserved or not? &  Surveillance as sensitivity criteria? & Data integrity preserved or not? & User input & Region tracking\\\hline
			
		\end{tabular}
\normalsize 
\end{table*}

